Hierarchical b-Matching

A matching of a graph is a subset of edges no two of which share a common vertex, and a maximum matching is a matching of maximum cardinality. In a $b$-matching every vertex $v$ has an associated bound $b_v$, and a maximum $b$-matching is a maximum set of edges, such that every vertex $v$ appears in at most $b_v$ of them. We study an extension of this problem, termed {\em Hierarchical b-Matching}. In this extension, the vertices are arranged in a hierarchical manner. At the first level the vertices are partitioned into disjoint subsets, with a given bound for each subset. At the second level the set of these subsets is again partitioned into disjoint subsets, with a given bound for each subset, and so on. In an {\em Hierarchical b-matching} we look for a maximum set of edges, that will obey all bounds (that is, no vertex $v$ participates in more than $b_v$ edges, then all the vertices in one subset do not participate in more that that subset's bound of edges, and so on hierarchically). We propose a polynomial-time algorithm for this new problem, that works for any number of levels of this hierarchical structure.

==> Mordo.tex <==
% ----------------------------------------------------------------
\vfuzz2pt % Don't report over-full v-boxes if over-edge is small
\hfuzz2pt % Don't report over-full h-boxes if over-edge is small
% THEOREMS -------------------------------------------------------
\usepackage{amsmath}
\usepackage{amssymb}

%\newenvironment{proof}{\noindent{\bf Proof:}}
%{\begin{flushright} \vspace{-0.5cm} $\square$ \end{flushright}}

%\newenvironment{sketch}{\noindent{\it Sketch of proof:}}
%{\begin{flushright} \vspace{-0.5cm} $\square$ \end{flushright}}
%\newcommand {\qed}{}

\newcommand {\npc}     {\textsc{NP}\textrm{-complete}}
\newcommand {\nph}     {\textsc{NP}\textrm{-hard}}
\newcommand {\apxh}     {\textsc{APX}\textrm{-hard}}
\newcommand {\fpt}     {\textsc{FPT}}
\newcommand {\wonehard}  {\textsc{W}[1]\textrm{-hard}}
\newcommand {\hyp}     {\textsc{P} \neq \textsc{NP}}
\newcommand {\nohyp}   {\textsc{P}=\textsc{NP}}
\newcommand {\bigoh}   {{\cal O}}

\newcommand {\runningtitle}[1] {\vspace{0.5ex}\noindent{\textbf{\boldmath #1:}}\\}
\newcommand {\runningtitleindent}[1] {\vspace{0.5ex}{\textbf{\boldmath #1:}}\\}

% MATH -----------------------------------------------------------
\newcommand {\norm}[1]{\left\Vert#1\right\Vert}
\newcommand {\abs}[1]{\left\vert#1\right\vert}
\newcommand {\set}[1]{\left\{#1\right\}}
\newcommand {\comb}[2]{\left(\begin{array}{c}#1 \\ #2 \end{array} \right)}
\newcommand {\defined} {\stackrel{def} {=}}
\newcommand {\isgeq} {\stackrel{?}{\geq}}
\newcommand {\isleq} {\stackrel{?}{\leq}}
% ----------------------------------------------------------------

